Evaluating the Smooth Control of Attribute Intensity in Text Generation with LLMs

Controlling the attribute intensity of text generation is crucial across scenarios (e.g., writing conciseness, chatting emotion, and explanation clarity). The remarkable capabilities of large language models (LLMs) have revolutionized text generation, prompting us to explore such \emph{smooth control} of LLM generation. Specifically, we propose metrics to assess the range, calibration, and consistency of the generated text's attribute intensity in response to varying control values, as well as its relevance to the intended context. To quantify the attribute intensity and context relevance, we propose an effective evaluation framework leveraging the Elo rating system and GPT4, both renowned for their robust alignment with human judgment. We look into two viable training-free methods for achieving smooth control of LLMs: (1) Prompting with semantic shifters, and (2) Modifying internal model representations. The evaluations of these two methods are conducted on $5$ different attributes with various models. Our code and dataset can be obtained from \url{https://github.com/ShangDataLab/Smooth-Control}.

==> tables/attributes_examples.tex <==
\begin{tabularx}{\textwidth}{l|*{5}{>{\raggedright\arraybackslash}X}} 
\hline
Degree & \anger & \happiness & \formality & \understandability & \conciseness \\
\hline
High & I have been simmering in outrage \ldots & My heart was soaring with joy \ldots &  &  &  \\ 
\hline
Low & The timing of your refund indeed stirs gentle curiosity \ldots & Despite the ample preparation and effort \ldots & & &  \\ 
\hline
\end{tabularx}

==> tables/main-table.tex <==
\begin{table*}[!t]
  \centering
   \small
    \begin{adjustbox}{max width=1\linewidth}
    {
        \begin{tabular}{c|c|cccccc|cccccc}
        \toprule
              & & \multicolumn{6}{c|}{\textbf{Attribute Intensity}} & \multicolumn{6}{c}{\textbf{Response Relevance}} \\
        \textbf{Method} & \textbf{Attr.} & \textbf{mistral} & \textbf{llama} & \textbf{llama-13b} & \textbf{llama-70b} & \textbf{gpt-3.5} & \textbf{gpt-4} & \textbf{mistral-7b} & \textbf{llama-7b} & \textbf{llama-13b} & \textbf{llama-70b} & \textbf{gpt-3.5} & \textbf{gpt-4} \\
        & & 7b & 7b \\
        \midrule
        \multirow{5}{*}{Prompt*} 
		& \textbf{\underline{A}}  & $3.12$ & $2.18$ & $2.05$ & $3.16$ & $2.10$ &           $2.32$ & $0.78$ & $0.75$ & $0.86$ & $0.72$ & $0.92$ & $0.99$ \\
		& \textbf{\underline{H}}  & $2.74$ & $1.77$ & $1.74$ & $2.19$ & $2.19$ &           $2.85$ & $0.81$ & $0.87$ & $0.94$ & $0.87$ & $1.00$ & $0.99$ \\
		& \textbf{\underline{F}}  & $2.64$ & $2.70$ & $2.57$ & $2.73$ & $2.51$ &           $2.40$ & $0.75$ & $0.95$ & $0.99$ & $0.91$ & $0.96$ & $0.99$ \\
		& \textbf{\underline{U}}  & $5.02$ & $3.21$ & $3.33$ & $4.76$ & $6.12$ &           $3.43$ & $0.45$ & $0.81$ & $0.83$ & $0.91$ & $0.86$ & $0.93$ \\
		& \textbf{\underline{C}}  & $4.26$ & $3.79$ & $3.28$ & $3.33$ & $4.54$ &           $3.77$ & $0.77$ & $0.92$ & $0.93$ & $0.91$ & $0.89$ & $1.00$ \\
        \midrule
        \multirow{5}{*}{Prompt} 
		& \textbf{\underline{A}}  & $2.02$ & $1.65$ & $1.65$ & $2.87$ & $1.79$ &           $1.76$ & $0.79$ & $0.79$ & $0.91$ & $0.83$ & $1.00$ & $0.99$ \\
		& \textbf{\underline{H}}  & $2.55$ & $1.60$ & $1.46$ & $1.92$ & $1.98$ &           $2.03$ & $0.83$ & $0.90$ & $0.92$ & $0.90$ & $1.00$ & $0.99$ \\
		& \textbf{\underline{F}}  & $2.48$ & $2.32$ & $2.15$ & $2.26$ & $2.20$ &           $1.83$ & $0.75$ & $0.97$ & $1.00$ & $0.93$ & $0.96$ & $0.99$ \\
		& \textbf{\underline{U}}  & $5.30$ & $3.06$ & $3.01$ & $2.96$ & $4.66$ &           $1.98$ & $0.72$ & $0.84$ & $0.91$ & $0.88$ & $0.95$ & $0.99$ \\
		& \textbf{\underline{C}}  & $3.91$ & $3.58$ & $3.28$ & $3.00$ & $3.96$ &           $3.02$ & $0.76$ & $0.95$ & $0.93$ & $0.90$ & $0.98$ & $1.00$ \\
        \midrule
        \multirow{5}{*}{RepE} 
		& \textbf{\underline{A}}  & $3.70$ & $3.67$ & $2.79$ & $--$ & $--$ & $--$ & $0.81$ & $0.93$ & $0.95$ & $--$ & $--$ & $--$ \\
		& \textbf{\underline{H}}  & $3.18$ & $3.58$ & $3.45$ & $--$ & $--$ & $--$ & $0.80$ & $0.87$ & $0.93$ & $--$ & $--$ & $--$ \\
		& \textbf{\underline{F}}  & $3.27$ & $3.66$ & $3.30$ & $--$ & $--$ & $--$ & $0.93$ & $0.82$ & $0.94$ & $--$ & $--$ & $--$ \\
		& \textbf{\underline{U}}  & $3.93$ & $4.25$ & $2.56$ & $--$ & $--$ & $--$ & $0.97$ & $0.88$ & $0.72$ & $--$ & $--$ & $--$ \\
		& \textbf{\underline{C}}  & $2.78$ & $2.98$ & $3.09$ & $--$ & $--$ & $--$ & $0.95$ & $0.97$ & $0.67$ & $--$ & $--$ & $--$ \\
        \bottomrule
        \end{tabular}
    }
    \end{adjustbox}
    \caption{Experimental Results for Training (Selected 10 from 20)}
  \label{tab:exp_baseline}%
\end{table*}



\begin{table*}[!t]
  \centering
   \small
    \begin{adjustbox}{max width=1\linewidth}
    {
        \begin{tabular}{c|c|cccccc|cccccc}
        \toprule
              & & \multicolumn{6}{c|}{\textbf{Calibration}} & \multicolumn{6}{c}{\textbf{Variance}} \\
        \textbf{Method} & \textbf{Attribute} & \textbf{mistral-7B} & \textbf{llama-7B} & \textbf{llama-13B} & \textbf{llama-70B} & \textbf{gpt-3.5} & \textbf{gpt-4} & \textbf{mistral-7B} & \textbf{llama-7B} & \textbf{llama-13B} & \textbf{llama-70B} & \textbf{gpt-3.5} & \textbf{gpt-4} \\
        \midrule
        \multirow{5}{*}{Prompt} 
            & \textbf{\underline{A}}              & $1.94$ & $1.08$ & $0.84$ & $1.49$ & $0.86$ & $0.85$ & $1.17$ & $1.10$ & $1.20$ & $1.67$ & $1.23$ & $1.47$ \\
            & \textbf{\underline{H}}          & $1.26$ & $0.51$ & $0.50$ & $0.96$ & $0.77$ & $1.25$ & $1.48$ & $1.25$ & $1.23$ & $1.23$ & $1.42$ & $1.60$ \\
            & \textbf{\underline{F}}         & $1.46$ & $1.48$ & $1.54$ & $1.50$ & $1.36$ & $1.29$ & $1.19$ & $1.23$ & $1.03$ & $1.23$ & $1.16$ & $1.12$ \\
            & \textbf{\underline{U}}        & $3.35$ & $1.65$ & $1.70$ & $2.68$ & $4.03$ & $2.30$ & $1.67$ & $1.56$ & $1.63$ & $2.08$ & $2.09$ & $1.12$ \\
            & \textbf{\underline{C}}  & $1.60$ & $1.08$ & $1.30$ & $0.90$ & $3.19$ & $1.63$ & $2.66$ & $2.71$ & $1.98$ & $2.43$ & $1.36$ & $2.13$ \\
        \midrule
        \multirow{5}{*}{Prompt} 
            & \textbf{\underline{A}}             & $0.87$ & $0.63$ & $0.72$ & $1.50$ & $0.63$ & $0.51$ & $0.83$ & $0.97$ & $0.68$ & $0.87$ & $0.93$ & $1.03$ \\
            & \textbf{\underline{H}}          & $1.07$ & $0.42$ & $0.32$ & $0.66$ & $0.58$ & $0.45$ & $1.34$ & $1.03$ & $0.82$ & $0.92$ & $1.02$ & $1.33$ \\
            & \textbf{\underline{F}}          & $1.33$ & $1.08$ & $1.24$ & $1.21$ & $1.14$ & $0.73$ & $1.47$ & $1.19$ & $0.90$ & $1.10$ & $1.06$ & $1.07$ \\
            & \textbf{\underline{U}}        & $3.70$ & $1.55$ & $1.63$ & $0.70$ & $1.89$ & $0.69$ & $1.73$ & $1.52$ & $1.47$ & $2.34$ & $2.77$ & $1.06$ \\
            & \textbf{\underline{C}}  & $1.30$ & $1.11$ & $1.30$ & $0.73$ & $2.36$ & $0.79$ & $3.59$ & $3.62$ & $2.68$ & $4.94$ & $1.62$ & $3.41$ \\
        \midrule
        \multirow{5}{*}{RepE} 
            & \textbf{\underline{A}}              & $1.94$ & $1.33$ & $1.32$ &  $--$ & $--$ & $--$ & $0.87$ & $1.22$ & $1.13$ & $--$ & $--$ & $--$ \\
            & \textbf{\underline{H}}          & $1.18$ & $1.52$ & $1.68$ & $--$ & $--$ & $--$ & $2.14$ & $2.10$ & $1.92$ & $--$ & $--$ & $--$ \\
            & \textbf{\underline{F}}          & $1.86$ & $2.06$ & $1.90$ & $--$ & $--$ & $--$ & $1.44$ & $1.50$ & $1.59$ & $--$ & $--$ & $--$ \\
            & \textbf{\underline{U}}        & $2.08$ & $2.29$ & $0.58$ & $--$ & $--$ & $--$ & $1.75$ & $2.02$ & $2.07$ & $--$ & $--$ & $--$ \\
            & \textbf{\underline{C}}  & $1.26$ & $1.40$ & $1.39$ & $--$ & $--$ & $--$ & $0.92$ & $0.76$ & $0.90$ & $--$ & $--$ & $--$ \\
        
        \bottomrule
        \end{tabular}
    }
    \end{adjustbox}
    \caption{Decomposed Evaluation of Attribute Intensity for Training (Selected 10 from 20)}
  \label{tab:exp_baseline}%
\end{table*}


==> tables/model-unknown-shifter.tex <==
\begin{table*}[!t]
  \centering
   \small
    \begin{adjustbox}{max width=1\linewidth}
    {
        \begin{tabular}{c|c|cccccc|cccccc|cccccc}
        \toprule
        & 
        & \multicolumn{6}{c|}{\textbf{Calibration}\chengyu{copy results}} 
        & \multicolumn{6}{c}{\textbf{Variance}\chengyu{copy results}}
        & \multicolumn{6}{c}{\textbf{Relevance}} \\
        \textbf{Method} & \textbf{Attr.} 
        % & \textbf{mistral} & \textbf{llama} & \textbf{llama-13b} & \textbf{llama-70b} & \textbf{gpt-3.5} & \textbf{gpt-4} 
        % & \textbf{mistral-7b} & \textbf{llama-7b} & \textbf{llama-13b} & \textbf{llama-70b} & \textbf{gpt-3.5} & \textbf{gpt-4}
        % & \textbf{mistral-7b} & \textbf{llama-7b} & \textbf{llama-13b} & \textbf{llama-70b} & \textbf{gpt-3.5} & \textbf{gpt-4} \\
        % & & 7b & 7b \\
        \\
        \midrule
        \multirow{5}{*}{Prompt*} 
		& \textbf{\underline{A}} 
        & $3.12$ & $2.18$ & $2.05$ & $3.16$ & $2.10$ &  $2.32$ 
        & $0.78$ & $0.75$ & $0.86$ & $0.72$ & $0.92$ & $0.99$ 
        & $0.78$ & $0.75$ & $0.86$ & $0.72$ & $0.92$ & $0.99$ \\
		& \textbf{\underline{H}}  & $2.74$ & $1.77$ & $1.74$ & $2.19$ & $2.19$ &           $2.85$ & $0.81$ & $0.87$ & $0.94$ & $0.87$ & $1.00$ & $0.99$ \\
		& \textbf{\underline{F}}  & $2.64$ & $2.70$ & $2.57$ & $2.73$ & $2.51$ &           $2.40$ & $0.75$ & $0.95$ & $0.99$ & $0.91$ & $0.96$ & $0.99$ \\
		& \textbf{\underline{U}}  & $5.02$ & $3.21$ & $3.33$ & $4.76$ & $6.12$ &           $3.43$ & $0.45$ & $0.81$ & $0.83$ & $0.91$ & $0.86$ & $0.93$ \\
		& \textbf{\underline{C}}  & $4.26$ & $3.79$ & $3.28$ & $3.33$ & $4.54$ &           $3.77$ & $0.77$ & $0.92$ & $0.93$ & $0.91$ & $0.89$ & $1.00$ \\
        \bottomrule
        \end{tabular}
    }
    \end{adjustbox}
    \caption{Performance of intensity calibration that is universal to model}
  \label{tab:exp-unknown-model}%
\end{table*}



